Causal Markov Decision Processes: Learning Good Interventions Efficiently

We introduce causal Markov Decision Processes (C-MDPs), a new formalism for sequential decision making which combines the standard MDP formulation with causal structures over state transition and reward functions. Many contemporary and emerging application areas such as digital healthcare and digital marketing can benefit from modeling with C-MDPs due to the causal mechanisms underlying the relationship between interventions and states/rewards. We propose the causal upper confidence bound value iteration (C-UCBVI) algorithm that exploits the causal structure in C-MDPs and improves the performance of standard reinforcement learning algorithms that do not take causal knowledge into account. We prove that C-UCBVI satisfies an $\tilde{O}(HS\sqrt{ZT})$ regret bound, where $T$ is the the total time steps, $H$ is the episodic horizon, and $S$ is the cardinality of the state space. Notably, our regret bound does not scale with the size of actions/interventions ($A$), but only scales with a causal graph dependent quantity $Z$ which can be exponentially smaller than $A$. By extending C-UCBVI to the factored MDP setting, we propose the causal factored UCBVI (CF-UCBVI) algorithm, which further reduces the regret exponentially in terms of $S$. Furthermore, we show that RL algorithms for linear MDP problems can also be incorporated in C-MDPs. We empirically show the benefit of our causal approaches in various settings to validate our algorithms and theoretical results.

==> regret.tex <==
\begin{thm} \label{thm:CUCBVI}
	Consider $\delta>0$, the regret of C-UCBVI (Algorithm~\ref{algo:CUCBVI}) is bounded by:
	\begin{align}
		R_K = \tilde{O}\left(H^2S\sqrt{|\mathcal{Z}|T}+H^2S^2|\mathcal{Z}|\right),
	\end{align}
	with probability at least $1-\delta$.
	
	\textcolor{red}{Replacing the bonus term by $b(x,\mathbf{Z}) = 7HL\sqrt{\frac{S}{N_k(x,\mathbf{Z})}}$ and using Weissman theorem on the estimation error of transition probabilities (1-norm), one can achieve final regret $R_K = \tilde{O}\left(HS\sqrt{|\mathcal{Z}|T}\right)$}
\end{thm}

Our result drops the dependence from $A$ to $|\mathcal{Z}|$.

\textcolor{red}{Add more conclusion here.}

==> sketch.tex <==
We follow the proof idea of UCBVI to bound the cumulative regret. And in each part of the proof, we utilize the causal structures and certain causal related probabilities. We present the proof sketch for eight key steps in this section and leave some technical proofs deferred to the appendix for a cleaner presentation. Throughout the sketch and detailed proofs in the appendix, we define the logarithmic term by $L:=\log\left(CH|\mathcal{Z}|ST/\delta\right)$, where $C$ is a large enough constant.

The regret of C-UCBVI up to episode $K$ is defined by:
\begin{align*}
	R_K = \sum_{k=1}^{K}\left(V_1^*(x_{k,1})-V_1^{\pi_k}(x_{k,1})\right).
\end{align*}
Define the value function difference terms at level $h$ in episode $k$ by $\Delta_{k,h}:=V_h^*-V_h^{\pi_k}$ and $\widetilde{\Delta}_{k,h}:=V_{k,h}-V_h^{\pi_k}$. Define their realizations at state $x_{k,h}$ by $\delta_{k,h}:=\Delta_{k,h}(x_{k,h})$ and $\widetilde{\delta}_{k,h}:=\widetilde{\Delta}_{k,h}(x_{k,h})$. Under these notations, the regret can be written as:
\begin{align*}
	R_K = \sum_{k=1}^{K}\delta_{k,1}.
\end{align*}

At first step, we show that the optimism property, i.e. $V_{k,h}(x)$ terms upper bound the optimal value functions $V_h^*(x)$ for all $(k,h,x)$ tuples, holds with high probability. Since we have no knowledge on the optimal value functions appearing as a key term in regret, it is hard to directly bound terms $\delta_{k,1}$. Claim~\ref{claim:UCB} shows that we can instead bound $\tilde{\delta}_{k,1}$, which depends mostly on the information provided by the algorithm.
\begin{claim} [Optimism]\label{claim:UCB}
	Define optimism events as follows:
	\begin{align*}
		\mathcal{G}=\{V_{k,h}(x)\geq V_h^*(x), \forall k,h,x\},
	\end{align*}
	we have $P(\mathcal{G})\geq 1-\delta$.
\end{claim}
This can be proved by backward induction over $h$ for every $k$ showing that $\{q_{k,h}(x,\mathbf{Z})\geq q_h^*(x,\mathbf{Z}),\forall k,h,x,\mathbf{Z}\}$ holds with high probability. By the construction way of $Q_{k,h}$ functions in algorithm~\ref{algo:CUCBVI}, claim~\ref{claim:UCB} can then be proved using definitions value functions $q,Q$ and $V$.

According to claim~\ref{claim:UCB}, the regret is bounded by:
\begin{align*}
	R_K = \sum_{k=1}^{K}\delta_{k,1} \leq \sum_{k=1}^{K}\widetilde{\delta}_{k,1}.
\end{align*}

In order to divide each $\widetilde{\delta}_{k,1}$ into several pieces, we bound every $\widetilde{\delta}_{k,h}$ in a recursion way in terms of $\widetilde{\delta}_{k,h+1}$ showing in claim~\ref{claim:deltarecursive}.

\begin{claim}\label{claim:deltarecursive}
	Define the estimated state transition probabilities, weighted exploration bonus term using causal graph probabilities and martingale differences as below:
	\begin{align*}
		&\hat{P}_{k,h}^{\pi_k}(y|x)\\
		:=&\sum_{\mathbf{Z}\in\mathcal{Z}}\hat{P}_k(y|x_{k,h},\mathbf{Z})P(\text{Pa}_Y=\mathbf{Z}|x_{k,h},\pi_k(x_{k,h},h))\\
		b_{k,h}&:= \sum_{\mathbf{Z}}b_{k,h}(x_{k,h},\mathbf{Z}) P(\text{Pa}_Y=\mathbf{Z}|x_{k,h},\pi_k(x_{k,h},h))\\
		\epsilon_{k,h} &:= P_h^{\pi_k}\widetilde{\Delta}_{k,h+1}-\widetilde{\Delta}_{k,h+1}(x_{k,h+1})\\
		\varepsilon_{k,h} &:= \epsilon_{k,h}(x_{k,h}),
	\end{align*}
	where we set $\hat{P}_k(y|x_{k,h},\mathbf{Z}) = 0$ and $b_{k,h}(x_{k,h},\mathbf{Z}) = H$ when $N(x_{k,h},\mathbf{Z}) = 0$.
	$\widetilde{\delta}_{k,h}$ can be bounded as follows:
	\begin{align}
		\tilde{\delta}_{k,h}&\leq \widetilde{\delta}_{k,h+1}+\varepsilon_{k,h}+b_{k,h}+\left[(\hat{P}_{k,h}^{\pi_k}-P_{h}^{\pi_k})V_{h+1}^*\right](x_{k,h}) \notag\\
		&+\left[(\hat{P}_{k,h}^{\pi_k}-P_{h}^{\pi_k})(V_{k,h+1}-V_{h+1}^*)\right](x_{k,h}).
	\end{align}
\end{claim}

We now bound the last two terms in the result of claim~\ref{claim:deltarecursive}. The first term represents the error term in estimating the state transition probabilities applied on the optimal value function under policy $\pi_k$. 


\begin{claim} \label{claim:errorterm}
	For $\delta>0$, with probability at least $1-\delta$, the error term can be bounded by:
	\begin{align*}
		&\left|(\hat{P}_{k,h}^{\pi_k}-P_{h}^{\pi_k})V_{h+1}^*(x_{k,h})\right|\\
		\leq& \sum_{\mathbf{Z}:N_k(x_{k,h},\mathbf{Z})>0} P(\text{Pa}_Y=\mathbf{Z}|x_{k,h},\pi_k(x_{k,h}))\\
		\times& \left(\sqrt{\frac{2\mathbb{V}_h^*(x_{k,h},\mathbf{Z})L}{N_k(x_{k,h},\mathbf{Z})}}
		+\frac{2HL}{3N_k(x_{k,h},\mathbf{Z})}\right)\\
		+&H\sum_{\mathbf{Z}:N_k(x_{k,h},\mathbf{Z})=0}P(\text{Pa}_Y=\mathbf{Z}|x_{k,h},\pi_k(x_{k,h},h)),
	\end{align*}
	where $\mathbb{V}_h^*(x,\mathbf{Z}):=\text{Var}_{y\sim P(y|x,\mathbf{Z})} V_{h+1}^*(y)$.
\end{claim}

Claim~\ref{claim:errorterm} bounds the error term by two parts. The first part includes parent value assignments $\mathbf{Z}$ such that $N_k(x_{k,h},\mathbf{Z})>0$, which can be bound by Bernstein inequality with a union bound over $N_k(x_{k,h},\mathbf{Z})>0$. However, the challenge in our causal approach here is that there exists some $\mathbf{Z}$ never appearing together with state $x_{k,h}$, i.e. $N_k(x_{k,h},\mathbf{Z})=0$. We will analyze this part separately (second term in the bound of claim~\ref{claim:errorterm}) later, showing that such events cannot happen frequently. If one sums these terms over $k\in[K]$ and $h\in[H]$, the overall summation will not scale with $T=KH$.

Next, we bound the last term (higher order error term) in equation~\ref{equ:recursion} in claim~\ref{claim:correctionterm}. Following the proof idea of~\cite{azar2017minimax}, for every $(k,x,\mathbf{Z})$ tuple, we define two categories of states: typical/non-typical in equation~\ref{equ:typical}. Together with Bernstein's inequality, we achieve the bound in claim~\ref{claim:correctionterm}.

\begin{claim}\label{claim:correctionterm}
	For every $(x,\mathbf{Z})\in\mathcal{S}\times\mathcal{Z}$ the set of typical next states at every episode $k$ as follows:
	\begin{align} \label{equ:typical}
	[y]_{k,x,\mathbf{Z}}:=\{y:y\in\mathcal{S},N_k(x,\mathbf{Z})P(y|x,\mathbf{Z})\geq H^2L\},
	\end{align}
	then $\delta>0$, with probability at least $1-\delta$, one can show that:
	\begin{align*}
	&\left|\left((\hat{P}_{k,h}^{\pi_k}-P_{h}^{\pi_k})(V_{k,h+1}-V_{h+1}^*)\right)(x_{k,h})\right|\\
	\leq & 2\sqrt{L}\sum_{\mathbf{Z}:N_k(x_{k,h},\mathbf{Z})>0}P(\text{Pa}_Y=\mathbf{Z}|x_{k,h},\pi_k(x_{k,h},h))\\
	\times&\left(\bar{\varepsilon}_{k,h,\mathbf{Z}}+\sqrt{\frac{1}{H^2L}}\widetilde{\delta}_{k,h+1}+\frac{SH\sqrt{LH^2}}{N_k(x_{k,h},\mathbf{Z})}\right)\\
	+& 4SHL\sum_{\mathbf{Z}:N_k(x_{k,h},\mathbf{Z})>0}P(\text{Pa}_Y=\mathbf{Z}|x_{k,h},\pi_k(x_{k,h},h))\frac{1}{3N_k(x_{k,h},\mathbf{Z})}\\
	+&H\sum_{\mathbf{Z}:N_k(x,\mathbf{Z})=0}P(\text{Pa}_Y=\mathbf{Z}|x_{k,h},\pi_k(x_{k,h},h)),
	\end{align*}
	where 
	\begin{align*}
	\bar{\varepsilon}_{k,h,\mathbf{Z}}:=&\sum_{y\in\mathcal{S}} P(y|x_{k,h},\mathbf{Z})\sqrt{\frac{\mathbb{1}_{y\in[y]_{k,h,\mathbf{Z}}}}{N_k(x_{k,h},\mathbf{Z})P(y|x_{k,h},\mathbf{Z})}}\widetilde{\Delta}_{k,h+1}(y)\\
	& -\sqrt{\frac{1}{N_k(x_{k,h},\mathbf{Z})P(y|x_{k,h},\mathbf{Z})}}\mathbb{1}(y\in[y]_{k,h,\mathbf{Z}})\widetilde{\delta}_{k,h+1}.
	\end{align*} 
\end{claim}

Now combining the bounds for all terms showing in equation~\ref{equ:recursion}, we can bound every $\widetilde{\delta}_{k,h}$ term in claim~\ref{claim:deltabound} non-recursively.

\begin{claim} \label{claim:deltabound}
	Combine previous claims with inductions, one can show that:
	\begin{align*}
	&\widetilde{\delta}_{k,h}\\
	\leq& \sum_{j=h}^{H}2e\left(\varepsilon_{k,j}+b_{k,j}\right)\\
	+&\sum_{j=h}^{H}\sum_{\mathbf{Z}}2eP(\text{Pa}_Y=\mathbf{Z}|x_{k,j},\pi_k(x_{k,j},j))\\
	&\times\left(c_{k,j,\mathbf{Z}}+2\sqrt{L}\bar{\varepsilon}_{k,j,\mathbf{Z}}+\frac{2H^2SL}{N_k(x_{k,j},\mathbf{Z})}\right)\\
	+&2eH\sum_{j=h}^{H}\sum_{\mathbf{Z}:N_k(x_{k,h},\mathbf{Z})=0}P(\text{Pa}_Y=\mathbf{Z}|x_{k,h},\pi_k(x_{k,h},h)),
	\end{align*}
	where $c_{k,j,\mathbf{Z}} = \sqrt{\frac{2H^2\log(T/\delta)}{N_k(x_{k,j},\mathbf{Z})}}+\frac{2H\log(T/\delta)}{3N_k(x_{k,j},\mathbf{Z})}$.
\end{claim}

We now bound above several terms. 
\begin{claim} \label{claim:exploration}
	Bounding the sum of exploration terms $b_{k,h}$: for $\delta>0$, with probability at least $1-\delta$ we have:
	\begin{align*}
	\sum_{i=1}^{K}\sum_{j=1}^{H}b_{i,j} =  \tilde{O}\left(H\sqrt{S|\mathcal{Z}|T}+HS|\mathcal{Z}|\right).
	\end{align*}
\end{claim}

\begin{claim}\label{claim:mtgle}
	Bounding the martingale differences: by Azuma's inequality, for $\delta>0$, with probability at least $1-\delta$, we have:
	\begin{align*}
		&\sum_{i=1}^{K}\sum_{j=1}^{H}\epsilon_{i,j} = \tilde{O}\left(H\sqrt{T}\right)\\
		&\sum_{i=1}^{K}\sum_{j=1}^{H}\sum_{\mathbf{Z}:N_i(x_{i,j},\mathbf{Z})>0}P(\text{Pa}_Y=\mathbf{Z}|x_{i,j},\pi_i(x_{i,j},j))\bar{\varepsilon}_{i,j,\mathbf{Z}} \\
		&= \tilde{O}(\sqrt{T})
	\end{align*}
\end{claim}

\begin{claim}\label{claim:remain}
	Bound the remaining terms: 
	\begin{align*}
		&\sum_{i=1}^{K}\sum_{j=1}^{H}\sum_{\mathbf{Z}:N_i(x_{i,j},\mathbf{Z})>0}P(\text{Pa}_Y=\mathbf{Z}|x_{i,j},\pi_i(x_{i,j},j))\\
		&\times\left(c_{i,j,\mathbf{Z}}+\frac{2H^2SL}{N_i(x_{i,j},\mathbf{Z})}\right)
		= \tilde{O}\left(H^2S\sqrt{|\mathcal{Z}|T}+H^2S^2|\mathcal{Z}|\right)\\
		&H\sum_{i=1}^{K}\sum_{j=1}^{H}\sum_{\mathbf{Z}:N_i(x_{i,j},\mathbf{Z})=0}P(\text{Pa}_Y=\mathbf{Z}|x_{i,j},\pi_i(x_{i,j},j))\\
		&= \tilde{O}\left(HS|\mathcal{Z}|+H\sqrt{T}\right).
	\end{align*}
\end{claim}
